Identifying Secure Operating Ranges for DER Control using Bilevel Optimization

Active distribution grids are accommodating an increasing number of controllable electric loads and distributed energy resources (DERs). A majority of these DERs are managed by entities other than the distribution utility, such as individual customers or third-party aggregators, who control the loads and DERs without consideration of any distribution grid constraints. This makes it challenging for a distribution system operator (DSO) to allow third-party aggregators and transmission operators to fully exploit the flexibility offered by these resources while also ensuring that distribution grid constraints such as voltage magnitude limits are not violated. In this paper, we develop a bilevel optimization-based framework to determine the aggregate power flexibility that can be obtained from an unbalanced distribution grid while ensuring that there is no disaggregation solution that leads to grid constraint violations. The results are a set of constraints and operating rules that are easy to communicate, and which provide the entities that procure flexibility from DERs (e.g. transmission operators or third-party aggregators) with the ability to freely implement their own disaggregation strategy without intervention from the DSO. The proposed approach is tested on two unbalanced distribution feeders and our simulation results indicate that it is possible to determine a wide range of aggregate power flexibility, as long as a simple set of rules for DER control activation are followed.

==> paper-positioning.tex <==
Introduction section:

FERC Order 2222 ordered ISOs to create a process that will guarantee electricity market access for aggregations of DERs. 
Such aggregations are typically controlled by
third-party aggregators (i.e., entities that are distinct from either transmission or distribution grid operators), and often involves control of a large number of small resources across a wide geographical area. 
Though such aggregators already exist [reference] and are active in e.g. markets for reserve provision, it is expected that the number of aggregators and the sizes of the DER populations they control will increase with continued adoption of DERs by consumers, including solar PV and electric vehicles [reference for projections if possible?].
This will be a benefit to transmission grid operators, who can leverage DER flexibility for grid services that are needed. However, as the amount of DER actuation within distribution grids increases, there is an increased risk of local constraint violations (e.g. violations of voltage magnitudes) at the distribution level. 
Thus, we need new procedures to accommodate the the use of DER aggregations for transmission grid in a way that does not jeopardize power quality or security of operations in the distribution grid. 
One option would be to represent the full distribution grid model and all individual devices within the market clearing model. However, this would require three-phase AC power flow modeling and maintaining accurate representations of thousands of devices (and their respective control modes) in each feeder, thus leading to prohibitive the computational cost.
To reduce computational complexity, it is widely agreed that we need methods to communicate limitations on DER actuation without sharing detailed information of the distribution feeder and individual devices. 
The goal of this paper is to determine an allowable range of flexibility around the current operating point that can be securely procured from DER aggregators. We assume that the aggregators control a population of DERs within a distribution feeder, and actuate these resources without knowledge or consideration of distribution grid constraints. 

There are numerous works in literature that consider the characterization of DER flexibility, both for individual devices [], across a population of devices [] and at the level of individual feeders []. The latter type of assessment has leveraged optimal power flow based approaches [], or identified aggregate flexibility based on the individual flexibility regions of the DERs using either polytopic projection [] or Minkowski sums []. When assessing the total range of flexibility that is available, many works assume that the DSO directly controls all DERs, i.e. the DSO acts as an aggregator and can leverage DER resources for the dual objectives of providing transmission grid services and managing internal constraints [], often under consideration of load uncertainty []. 
Other works model the interactions between end consumers and aggregators [] or between aggregators and ISOs []. More recently, there has been an increased interest in capturing interactions between DSOs and aggregators [], including methods that provide DSOs with the opportunity to change control signals from the aggregator that would lead to violations []. 
Other models assume that DERs are controlled by aggregators that are separate from the DSO, and determine an allowable flexibility range for individual DERs []. A drawback of this approach is that generating the flexibility regions involves prioritizing one DER over another, and also assumes that aggregators would be able to effectively control individual devices to remain within the range.



In this paper, we propose a new approach that also aims to assess a range of DER flexibility, while making slightly different (and in our opinion, more practical) assumptions regarding communication between the DSO, aggregator and ISO. 
Specifically, our method aims to help DSOs identify an allowable secure flexibility range around the current operating point. The input to the method is information regarding the distribution feeder parameters and (limited) information about the current operating state, as well as the location and technically possible range of set-points for individual DERs (this does not have to be real time information, but could be device characteristics provided by the aggregators when new devices enroll in their programs). The output of the method is an allowable flexibility range that determines upper and lower bounds on the total amount of flexibility that can securely be procured from DER aggregators active within the feeder. This range can be communicated to the ISO for inclusion in the market clearing, and can be interpreted as a simplified representation of distribution grid constraints. To obtain practical ranges of flexibility, we also need to incorporate some simple rules on DER actuation that aggregators need to follow. We also show that allowing the DSO to control reactive power significantly increases the amount of active power flexibility that DERs are allowed to provide. 

A key feature of the proposed approach is that it does not prescribe or limit which DERs that need to be providing flexibility, as long as the cumulative amount of actuation stays within the allowable range. Thus, the method places minimal limits on both how much flexibility should be procured from each of several aggregators that may be active within the feeder, and how aggregators choose to actuate the DERs that they control to achieve a certain set-point after they have been contracted to provide flexibility. 

Summary of contributions

Overview of remaining paper


Problem set-up section

- Example of what we are trying to do
- Discussion of some details on the problem set-up (maybe move something from above...? maybe move something from later in the paper? It would be good to make it clear who is controlling what and how these assumptions impact results...)
- Bilevel set-up (from original introduction? who decides what)
- Discussion of how all DERs have to move in the same direction (maybe move from current Sec. II.D 3?)
- Discussion of voltage control schemes



